Routing Oblivious Measurement Analytics

Network-wide traffic analytics are often needed for various network monitoring tasks. These measurements are often performed by collecting samples at network switches, which are then sent to the controller for aggregation. However, performing such analytics without ``overcounting'' flows or packets that traverse multiple measurement switches is challenging. Therefore, existing solutions often simplify the problem by making assumptions on the routing or measurement switch placement. We introduce AROMA, a measurement infrastructure that generates a uniform sample of packets and flows regardless of the topology, workload and routing. Therefore, AROMA can be deployed in many settings, and can also work in the data plane using programmable PISA switches. The AROMA infrastructure includes controller algorithms that approximate a variety of essential measurement tasks while providing formal accuracy guarantees. Using extensive simulations on real-world network traces, we show that our algorithms are competitively accurate compared to the best existing solutions despite the fact that they make no assumptions on the underlying network or the placement of measurement switches.

==> Extensions.tex <==
\section{Extensions}\label{sec:extensions}
Here we can talk about:
\begin{itemize}
\item Elephant flows (HH by volume). This should be doable using a ``weighted count distinct'' algorithm~\cite{WeightedCD} instead of HLL.
\item Other functions; e.g., unique counts.
\item Sliding windows; using a sliding window count distinct algorithm, e.g.~\cite{SlidingHLL,Fusy-HLL}
\item Hierarchal heavy hitters. Should be straight-forward. Perhaps we can also evaluate that. 
\item Supporting deletions. That is, if we assume that a router can know that it is the last measurement point, we can also find the amount of traffic that visited at least one router but has not reached it's destination.
\end{itemize} 

==> countMinSketchAlgs-old.tex <==
\section{Algorithms}\label{sec:algs}
In this section, we provide algorithms for the above problems. Our algorithms use a count distinct algorithm $\ALG$ as a black box. We assume that $\ALG$ allows processing of a stream and upon query provides a $(1+\epsilon_\ALG)$-approximation of the number of distinct items in the stream with probability $\ge 1-\delta_\ALG$.
We assume that \ALG{} supports three functions; \add{\cdot} processes elements, \query{} returns an estimate to the number of distinct elements,
and \merge{\ALG_1, \ALG_2} returns a merge of the instances $\ALG_1$ and $\ALG_2$. That is, assume that the sets of distinct elements observed by $\ALG_1$ and $\ALG_2$ are $S_1$ and $S_2$, then \merge{\ALG_1, \ALG_2} is an instance that monitors $S_1\cup S_2$. This property, which existing count distinct algorithms are known to have~\cite{}, is called as \emph{mergability}. We denote by $\algSize$ the space required by $S$; we note that a $\algSize=O\parentheses{\parentheses{\epsilon_\ALG^{-2}+\log  n}\log\delta_\ALG^{-1}}$ bits algorithm is known~\cite{woodruff} for $\le n$ distinct elements. Further, this algorithm processes new elements and answers queries in $O(1)$ time.
%, but is not efficient in practice~\cite{}. 
%Instead, we use the popular Hyper Log Log algorithm~\cite{} that requires $\algSize=O\parentheses{\parentheses{\epsilon_\ALG^{-2}\log\log n+\log n}\log\delta_\ALG^{-1}}$ space.
\subsection{\volEst{}}\label{sec:volEsT}
The problem of computing the overall amount of traffic is not trivial if packets may be measured on multiple hops along their route. If we assume that the routes are fixed and known in advance, we can partition the flows between routers such that each router measures flows that are not monitored in different places. Alas, routing may change over time and assigning responsibilities such that each flow will be monitored in exactly one point may be infeasible. 
Thus, we require a solution that tracks the overall number of packets without assumptions on the network topology, routing, or the order of packets.
For this, we propose using a count distinct algorithm $\ALG$ in each router. When a router handles a packet $\angles{x, i}$, it simply performs $\add{\angles{x, i}}$. Then, each router transmits his algorithm instance to the controller. The controller merges all instances to obtain a global view.
\begin{theorem}
Let $\epsilon_\ALG=\eps, \delta_\ALG=\delta$ be the parameters for the algorithm \ALG{} that runs on each router. Then the merged instances solves \paramVolEst{}.
\end{theorem}
\subsection{\freq{}}
Our solution is inspired by the Count-Min Sketch~\cite{CMSketch} while replacing each counter with an instance of $\ALG$.
Namely, we allocate a matrix of $d\times w$ instances of $\ALG$ in each router $R_r$. For $a\in\set{1,\ldots d}$ and $b\in\set{1,\ldots,w}$ we refer to the instance as $\ALG_{r,a,b}$.
 Additionally, each router uses $d$ pairwise-independent hash functions $h_r:\mathcal U\to \set{1,\ldots, w}$. It is crucial that all routers use the \emph{same} hash functions to allow aggregation.
The routers periodically send their data structure to a centralized controller that computes an aggregated, network-wide, view for serving queries.
Upon an arrival of a packet $\langle x,i\rangle$ at router $R_r$, it is added to $\mathbb{A}_{r,\ell,h_\ell(x)}$ for $\ell=1,\ldots d$.
A pseudo-code of our algorithm appears in Algorithm~\ref{alg:freq}.

\begin{algorithm}[h]
	\ifdefined \NINEPAGES
	\small
	\fi
	Initialization, at each router $r\in\set{1,\ldots,k}$:\\ $\hspace*{1cm}\forall a\in\set{1,\ldots d},b\in\set{1,\ldots,w}: \ALG_{r,a,b}.\mathit{init}(\epsilon_\ALG, \delta_\ALG)$
	\begin{algorithmic}[1]
\Function{Add$_r$}{Item $x$, sequence number $i$}\Comment{\footnotesize Runs at router $R_r$}
	\For {$\ell=1,2,\ldots,d$}
		\State $\mathbb{A}_{r,\ell,h_\ell(x)}.\mbox{\sc Add}(\langle x,i\rangle)$
	\EndFor
	\EndFunction
\Function{Merge}{$\set{\mathbb{A}_{r,a,b}}$}\Comment{\footnotesize Runs at the controller}
	\State $\forall a\in\set{1,\ldots d},b\in\set{1,\ldots,w}: \ALG_{c,a,b}.\mathit{init}(\epsilon_\ALG, \delta_\ALG)$
	\For {$r=1,2,\ldots,k$}
		\For {$a=1,2,\ldots,d$}		
			\For {$b=1,2,\ldots,w$}
				\State $\ALG_{c,a,b}\gets \mathit{Merge}\parentheses{\ALG_{c,a,b}, \mathbb{A}_{r,a,b}}$
			\EndFor
		\EndFor
	\EndFor
\EndFunction	
\Function{Query}{Item $x$}\Comment{\footnotesize Runs at the controller}
	\State \Return $\parentheses{1+2\epsilon_\ALG}\min_{\ell\in\set{1,\ldots, d}} \mathbb{A}_{c,\ell,h_\ell(x)}.\mbox{\sc Query}()$
\EndFunction	
	\end{algorithmic}
	\caption{\freq{}}
	\label{alg:freq}
\end{algorithm}
\normalsize
%\vspace*{-0.5cm}

In section~\ref{sec:analysis}, we prove the following theorem.
\begin{theorem}\label{thm:freqCorrectness}
	Assume that $\eps<1/2$ and let $\epsilon_\ALG=\eps/8, \delta_\ALG=\delta/2d, w=4/\epsilon, d=1+\log_2\delta^{-1}$ be the parameters for the algorithm \ALG{} that runs on each router. Then Algorithm~\ref{alg:freq} solves \paramFreq{}. The algorithm requires $O(\eps^{-1}\log\delta^{-1}\algSize)$ space, performs updates in $O(\log\delta^{-1})$ time and serves queries in time $O(\log\delta^{-1})$.
\end{theorem}

\subsection{\hhs{}}
Intuitively, one could use Algorithm~\ref{alg:freq} to solve \hhs{} by iterating over all $x\in\mathcal U$ and checking whether $\widehat{{f_x}}\ge |\mathcal S|\theta$. However, this approach is prohibitively slow as the universe size is large. For example, if $\mathcal U$ consists of all (srcip,dstip) pairs, one would need to iterate over more than $10^{18}$ identifiers. Thus, we require an alternative method.

A simple approach would be to keep a heap of potential heavy hitters on each switch and send it to the controller. However, in order to make sure that every heavy hitter appears at least on one such heap we may require a large amount of space. Namely, if each of a flow's packets arrive at a single router, and each router processes $|\mathcal S|\theta/k$ packets then the flow is a heavy hitters. However, this would mean that each heap size has to be $\Omega(k/\epsilon)$ if $\theta=O(\epsilon)$. This dictates that when additional routers are added to the network, one has to allocate the old ones with more space. Thus, this solution may not be scalable and an alternative that keeps the routers memory independent of $k$ is desired.

Thus, we adapt the \emph{hierarchical approach} for finding heavy hitters~\cite{CMS} to our settings. Intuitively, in a single-node measurement one can find the heavy hitters using a min-heap that store flow candidates. However, the Count Min Sketch operates at the more general \emph{strict turnstile} model in which elements may be deleted and not just added. In such setting, a heap does not allow one to find the heavy hitters as all of its flows may be deleted, leaving us with no information about the remaining large flows. Instead, a $O(\log|\mathcal U|)$ instances of the Count Min Sketch are used in parallel; whenever a packet arrives, all of its identifier \emph{prefixes} are inserted into the different instances.
In our setting, our router employs a hierarchy of Algorithm~\ref{alg:freq} instances.To get a network-wide view, the controller then merge all data structures obtained by the routers. For convenience, we denote by $\FREQALG$ an instance of Algorithm~\ref{alg:freq} initiated with $\eps_{\FREQALG}$ and $\eps_{\FREQALG}$.
To infer the heavy hitters from the prefix tree, we iteratively expand the prefixes using the functions $\mathit{descendants}_q(S)\triangleq\set{x\in\set{0,1}^{u-q}0^q\mid \parentheses{x\ \& \ 0^{q+1}}\in S}$; that is, given a set of $u-(q+1)$-bits heavy prefixes we consider all $u-q$ bits prefixes that are reached by adding either zero or one to a prefix in $S$.
The pseudo-code of our solution appears in Algorithm~\ref{alg:hhs}. For simplicity of presentation, we assume that $\mathcal U = \set{0,1,\ldots,2^u-1}$ and $u\triangleq \log_2|\mathcal U|\in\mathbb N$.
Additionally, and unlike the original hierarchy construction, we employ a \volEst{} algorithm. That is, differently than in a single node setting, we do not know the exact size of $\mathcal S$. Instead, we estimate $|\mathcal{S}|$ to within a $(1+\eps_s)$-multiplicative factor using the algorithm from Section~\ref{sec:volEsT}. Further, since distinct packets from different flows that share a prefix may have the same sequence number, we no longer have can treat each sequence number as a distinct identifier. Instead, given a packet $\angles{x,i}$ we treat it as if its serial number was $i\cdot x$ (a \emph{concatenation} of the sequence number and the identifier). This increases the size of the universe, as observed by \FREQALG{} to $|\mathcal U|\cdot n$, where $n\ge |\mathcal S|$ is the a bound on the overall number of packets.
Additionally, we show that our data structure allows answering \paramFreq{} queries in $O(1)$ time. That is, data structure of Algorithm~\ref{alg:hhs} serves faster frequency queries than Algorithm~\ref{alg:freq} but requires more space and update time.
Intuitively, our hierarchical data structure allows us to save a set of candidate heavy hitters (and their approximate frequencies) such that we are allows to estimate the frequency of any flow that is excluded from the set as zero.

%\begin{algorithm}[h]
%	\ifdefined \NINEPAGES
%	\small
%	\fi
%	Initialization, at each router $r\in\set{1,\ldots,k}$:\\ $\hspace*{1cm}\forall q\in\set{0,\ldots,u-1}: \FREQALG_{r,q}.\mathit{init}(\epsilon_\FREQALG, \delta_\FREQALG)
%%	; \ALG_r.\mathit{init}(\epsilon_\ALG, \delta_\ALG)$
%	$
%	\begin{algorithmic}[1]
%		\Function{Add$_r$}{Item $x$, sequence number $i$}\Comment{\footnotesize Runs at router $R_r$}
%%		\State $\FREQALG_{r,0}.\mbox{\sc Add}(x)$
%%		\State $\ALG_r.\mbox{\sc Add}(\langle x,i\rangle)$ \Comment{For estimating $|\mathcal S|$}
%		\For {$q=0,1,\ldots,u$}
%			\State $\mask \gets 11\ldots00$ \Comment{$q$ zeros, $u-q$ ones}
%			\State $\FREQALG_{r,q}.\mbox{\sc Add}(\langle x \& \mask,i\cdot x\rangle)$ \Comment{Bitwise-AND}
%		\EndFor
%		\EndFunction
%		\Function{Merge}{$\set{\FREQALG_{r,q}},\set{\ALG_r}$}\Comment{\footnotesize Runs at the controller}
%%		\State $\ALG_c.\mathit{init}(\epsilon_\ALG, \delta_\ALG)$ \Comment{The controller's instance for estimating $|\mathcal S|$}
%		\State $\forall q\in\set{0,\ldots,u}: \FREQALG_{c,q}.\mathit{init}(\epsilon_\FREQALG, \delta_\FREQALG)$
%		\For {$r=1,2,\ldots,k$}
%%		\State $\ALG_c\gets \mathit{Merge}\parentheses{\ALG_c,\ALG_r}$
%		\For {$q=0,1,\ldots,u$}		
%		\State $\FREQALG_{c,q}\gets \mathit{Merge}\parentheses{\FREQALG_{c,q}, \FREQALG_{r,q}}$
%		\EndFor
%		\EndFor
%		\EndFunction	
%		\Function{Query}{Threshold $\theta$}\Comment{\footnotesize Runs at the controller}
%		\State $\widehat{V} \gets \FREQALG_{c,u}.\mbox{\sc Query}(0\ldots 0)/(1+\epsilon_\FREQALG)$ \Comment{Estimate $|\mathcal S|$}
%		\State $T \gets \widehat{V}\theta$ \Comment{The reporting threshold}
%		\State $\mathit{HH_u}\gets\set{0\ldots 0}$\Comment{The root is always a heavy hitter}
%		\For {$q=u-1,u-2,\ldots,0$}		
%			\State $\hspace*{-0.2cm}\mathit{HH_q} \gets \set{x_q\in \mathit{descendants_q}(\mathit{HH_{q+1}})\mid\FREQALG_{c,q}.\mbox{\sc Query}(x_q)\ge T}$
%		\EndFor
%		\State \Return $\mathit{HH_0}$
%		\EndFunction	
%	\end{algorithmic}
%	\caption{OLD \hhs{}}
%	\label{alg:hhsOld}
%\end{algorithm}
%\normalsize

\begin{algorithm}[h]
	\ifdefined \NINEPAGES
	\small
	\fi
	Initialization, at each router $r\in\set{1,\ldots,k}$:\\ $\hspace*{1cm}\forall q\in\set{0,\ldots,u-1}: \FREQALG_{r,q}.\mathit{init}(\epsilon_\FREQALG, \delta_\FREQALG)
	%	; \ALG_r.\mathit{init}(\epsilon_\ALG, \delta_\ALG)$
	$
	\begin{algorithmic}[1]
		\Function{Add$_r$}{Item $x$, sequence number $i$}\Comment{\footnotesize Runs at router $R_r$}
		%		\State $\FREQALG_{r,0}.\mbox{\sc Add}(x)$
		%		\State $\ALG_r.\mbox{\sc Add}(\langle x,i\rangle)$ \Comment{For estimating $|\mathcal S|$}
		\For {$q=0,1,\ldots,u$}
		\State $\mask \gets \parentheses{\underbrace{11\ldots1}_{u-q}\underbrace{00\ldots0}_{q}}$ \Comment{$q$ zeros, $u-q$ ones}
		
		\State $\FREQALG_{r,q}.\mbox{\sc Add}(\langle x \& \mask,i\cdot x\rangle)$ \Comment{Bitwise-AND}
		\EndFor
		\EndFunction
		\Function{Merge}{$\set{\FREQALG_{r,q}},\set{\ALG_r}$}\Comment{\footnotesize Runs at the controller}
		%		\State $\ALG_c.\mathit{init}(\epsilon_\ALG, \delta_\ALG)$ \Comment{The controller's instance for estimating $|\mathcal S|$}
		\State $\forall q\in\set{0,\ldots,u}: \FREQALG_{c,q}.\mathit{init}(\epsilon_\FREQALG, \delta_\FREQALG)$
		\For {$r=1,2,\ldots,k$}
		%		\State $\ALG_c\gets \mathit{Merge}\parentheses{\ALG_c,\ALG_r}$
		\For {$q=0,1,\ldots,u$}		
		\State $\FREQALG_{c,q}\gets \mathit{Merge}\parentheses{\FREQALG_{c,q}, \FREQALG_{r,q}}$
		\EndFor
		\EndFor
		\State $\widehat{V} \gets \FREQALG_{c,u}.\mbox{\sc Query}(0\ldots 0)$ \Comment{Estimate $|\mathcal S|$}		
		\State $\mathit{TOP_u}\gets\set{0\ldots 0}$\label{line:inductionBasis}
		\For {$q=u-1,u-2,\ldots,0$}	\label{line:mergeFor}	
			\State $\hspace*{-0.2cm}\mathit{TOP_q} \gets \epsilon_\FREQALG^{-1}$ prefixes from $\mathit{descendants_q}(\mathit{TOP_{q+1}})$ with the largest estimations in $\FREQALG_{c,q}$\label{line:mergeTop}
		\EndFor
		\State $\mathit{HHCandidates} = \set{\angles{x,\widehat{{f_x}}}\mid x\in\mathit{TOP}_0}$\label{line:HHCandidates}\Statex\Comment{Store $\widehat{{f_x}}\triangleq\FREQALG_{c,0}.\mbox{\sc Query}(x)$ - the estimated frequency of $x$}
		\EndFunction	
		\Function{Query}{Threshold $\theta$}\Comment{\footnotesize Runs at the controller}
		\State $T \gets \widehat{V}\parentheses{\frac{\theta}{1+\epsilon_\FREQALG}-\epsilon_\FREQALG(1+\epsilon_\FREQALG)}$ \Comment{The reporting threshold}		
		\State \Return $\set{x\in\mathit{HHCandidates} | \widehat{{f_x}}\ge T}$
		\EndFunction
		\Function{FreqEst}{Item $x$}\Comment{\footnotesize Runs at the controller}
		\If {$x\in\mathit{HHCandidates}$}
			\State \Return $\widehat{{f_x}}$
		\Else
			\State \Return $0$
		\EndIf
		\EndFunction				
	\end{algorithmic}
	\caption{\hhs{}}
	\label{alg:hhs}
\end{algorithm}
\normalsize

We state the correctness of our algorithm here and defer the proof to Section~\ref{sec:analysis}.
\begin{theorem}\label{thm:hhsCorrectness}
	Assume that $\eps<1/2$ and denote  $\Psi\triangleq \eps^{-1}\log|\mathcal U|\log\delta^{-1}$; let $\epsilon_\FREQALG=\eps/2, \delta_\FREQALG=\Psi^{-1}$ be the parameters for the algorithm \FREQALG{} that runs on each router. Then Algorithm~\ref{alg:hhs} solves \hhs{}. The algorithm requires $O\parentheses{\eps^{-1}\log\delta^{-1}\log|\mathcal U|\log\Psi\parentheses{\eps^{-2}+\log n}}$ space, performs updates in $O(\log|\mathcal U|\log\Psi)$ time and serves queries in time $O(\eps^{-1}\log|\mathcal U|\log\Psi)$.
\end{theorem}

==> motivation.tex <==
\section{Motivation}
\red{To be removed.}
%{Danny work in progress...}
%TODO: preamble.

%Performing measurements in real-world networks is complicated due to frequent topology and routing change and rapidly changing traffic matrix.
%We want \sysName to achieve the following goals:

%\textbf{Generic measurement tool.} 
%\sysName should support various measurement queries over the packets / flows in the network, without assuming prior knowledge of the traffic distribution, and without conforming to only queries of a particular form.

%\textbf{Routing Oblivious.} 
%It's challenging to maintain accurate and timely knowledge of how packets are routed in the network. Instead, \sysName should work in a routing-oblivious fashion, producing accurate measurements regardless how packets traverse the network. 

%In particular, we can deploy \sysName in only a subset of the switches in the network to perform the measurement, as long as each packet goes through \emph{any} of the measurement switches.

%\textbf{Running on PISA programmable switches.}
%Today's commodity programmable switches ... (high speed, versatile)

%TODO: pisa constraint background.


%To the best of our knowledge, \sysName is the first system to achieve generic, routing-oblivious network measurement running on PISA programmable switches.
